TrackerSift: Untangling Mixed Tracking and Functional Web Resources

Trackers have recently started to mix tracking and functional resources to circumvent privacy-enhancing content blocking tools. Such mixed web resources put content blockers in a bind: risk breaking legitimate functionality if they act and risk missing privacy-invasive advertising and tracking if they do not. In this paper, we propose TrackerSift to progressively classify and untangle mixed web resources (that combine tracking and legitimate functionality) at multiple granularities of analysis (domain, hostname, script, and method). Using TrackerSift, we conduct a large-scale measurement study of such mixed resources on 100K websites. We find that more than 17% domains, 48% hostnames, 6% scripts, and 9% methods observed in our crawls combine tracking and legitimate functionality. While mixed web resources are prevalent across all granularities, TrackerSift is able to attribute 98% of the script-initiated network requests to either tracking or functional resources at the finest method-level granularity. Our analysis shows that mixed resources at different granularities are typically served from CDNs or as inlined and bundled scripts, and that blocking them indeed results in breakage of legitimate functionality. Our results highlight opportunities for finer-grained content blocking to remove mixed resources without breaking legitimate functionality.

==> graveyard.tex <==
Trackers and advertisers employ innovative techniques to circumvent content-blockers aiming to preserve user privacy.
%
 Content-blockers, such as uBlock Origin, frequently update filter lists to block tracking content in response to trackers evading filter lists by changing the network location of tracking content.
%
More recently, trackers start to mix tracking code resources with functional resources. Such practice prohibits content-blockers from restricting tracking activity at the code level without breaking legitimate functionality. 


In this paper, we conduct a large-scale measurement study to investigate the extent to which such circumvention practices have infiltrated today's web. 
%
We then propose a technique called \tool that progressively untangles web resources (i.e., tracking and functional) at four granularities: domain, hostname, script, and method.
%
Our measurement on the 100K websites finds 17\% of the total domains as mixed\textemdash domains that cater to both tracking and functional requests.
Among the mixed hostnames, \tool classifies 94\% of the JS scripts as either purely tracking or purely functional. In the remaining mixed JS scripts, \tool classifies 91\% of the JS methods successfully.
%
Our findings open new doors for effective, functionality-preserving content-blocking at a website's code level against sophisticated circumvention strategies such as varying content locations and mixed resources.





  \begin{table}[ht]
    \centering
    \caption{Results from Domain Level Analysis}
    \label{table: domain-results}
    \begin{tabular}{ |p{3cm}|p{1.3cm}|p{1.3cm}|  }
     \hline
     \multicolumn{3}{|c|}{Tracking Domains} \\
     \hline
     \vspace{0.6} \centering Domain  & \vspace{0.3} Tracking requests & Non-tracking requests\\
     \hline
            google-analytics.com & 43129 & 0 \\ 
           googlesyndication.com  & 24051 & 0 \\ 
           doubleclick.net & 33931& 255\\ 
           gnpge.com & 13639 & 0\\ 
           googleadservices.com & 6272 & 0\\ 
     \hline
  \end{tabular}
  
  \vspace{10}
  
  \begin{tabular}{ |p{3cm}|p{1.3cm}|p{1.3cm}|  }
     \hline
     \multicolumn{3}{|c|}{Non Tracking Domains} \\
     \hline
     \vspace{0.6} \centering Domain  & \vspace{0.3} Tracking requests & Non-tracking requests\\
     \hline
             twimg.com & 17 & 16856 \\ 
             zychr.com  & 6 & 1100 \\ 
             fbcdn.net & 1& 1051\\ 
             w.org & 0& 1049\\ 
             parastorage.com & 3& 976\\ 
     \hline
  \end{tabular}

 \vspace{10}
  
  \begin{tabular}{ |p{3cm}|p{1.3cm}|p{1.3cm}|  }
     \hline
     \multicolumn{3}{|c|}{Multipurpose Domains} \\
     \hline
     \vspace{0.6} \centering Domain  & \vspace{0.3} Tracking requests & Non-tracking requests\\
     \hline
             gstatic.com & 6238 & 28835 \\ 
             google.com & 18666 & 8870 \\ 
             facebook.com & 14620 & 3554 \\ 
             facebook.net & 12677 & 4389 \\ 
             wp.com & 2044 & 1550 \\  
     \hline
  \end{tabular}
\end{table}

  \begin{table}[ht]
    \centering
    \caption{Break down analysis for domain \textit{wp.com}}
    \label{table: wp.com-results}
    \begin{tabular}{ |p{3cm}|p{1.3cm}|p{1.3cm}|  }
     \hline
     \multicolumn{3}{|c|}{Tracking Host names} \\
     \hline
     \vspace{0.6} \centering Host name  & \vspace{0.3} Tracking requests & Non-tracking requests\\
     \hline
            pixel.wp.com & 1925 & 0 \\ 
           stats.wp.com  & 61 & 0 \\ 
     \hline
  \end{tabular}
  
  \vspace{10}
  
  \begin{tabular}{ |p{3cm}|p{1.3cm}|p{1.3cm}|  }
     \hline
     \multicolumn{3}{|c|}{Non Tracking Host names} \\
     \hline
     \vspace{0.6} \centering Host name  & \vspace{0.3} Tracking requests & Non-tracking requests\\
     \hline
             s0.wp.com & 0 & 73 \\ 
             c0.wp.com  & 0 & 177 \\ 
             i3.wp.com & 0& 2\\ 
             widgets.wp.com & 0& 82\\ 
     \hline
  \end{tabular}

 \vspace{10}
  
  \begin{tabular}{ |p{3cm}|p{1.3cm}|p{1.3cm}|  }
     \hline
     \multicolumn{3}{|c|}{Multipurpose Host names} \\
     \hline
     \vspace{0.6} \centering Host name  & \vspace{0.3} Tracking requests & Non-tracking requests\\
     \hline
             i1.wp.com & 12 & 362 \\ 
             i2.wp.com & 20 & 411 \\ 
             i0.wp.com & 26 & 443 \\ 
     \hline
  \end{tabular}
\end{table}




\begin{table}[ht]
    \centering
    \caption{Break down analysis for \textit{i1.wp.com}, \textit{i2.wp.com}, and \textit{i0.wp.com}  }
    \label{table: script-results}
    \begin{tabular}{ |p{1.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|  }
     \hline
     \vspace{3} Host name & Can be blocked on web pages &  Can not be blocked on web pages & \vspace{2} Total web pages\\
     \hline
         i1.wp.com & 115 & 5  & 120\\ 
         i2.wp.com & 130 & 6 & 136\\ 
         i0.wp.com & 127 & 7 & 134 \\ 
     \hline
  \end{tabular}
\end{table}



\gulzar{verbose, need to polish}
\textbf{Tracking-Inducing Resource Localization.} Inadvertently, the two research questions pose striking similarities with the traditional software engineering research on fault-inducing code localization. 
%
For example, widely popular spectra-based fault localization (SPFL)~\cite{} tests the software under investigation over a diverse set of test inputs and uses the collected statement coverage profiles of each test, passing or failing, to localize the lines of code that are most likely to induce a test failure. 
%
Our observation is that we can employ spectra-based fault localization techniques to classify resources in either advertising and tracking, which are analogous to failing tests, or functional, which is analogous to passing tests. 
%
However, a naive application of SPFL for such a classification raises two key concerns. 
%
First, SPFL's localizability is limited by the test suite's efficacy in capturing faulty behavior. In web applications, \emph{how do we correctly identify a tracking symptom?}
%
Second, SPFL performs intrusive instrumentation to capture statement-level coverage. 
%
For web pages, \emph{how do we efficiently collect such execution profile instead of naively instrumenting the runtime which can be prohibitively expensive?}. 
%
Addressing these challenges is vital for a precise and efficient investigation of the research questions. 

% One more thing, normally coverage for a test is either marked fail or pass. IN our case, we only have one profile.

% Add Fault localization intro and why that wouldn't work in this area. List possible limitations. state the limitations of finses grained fault isolation. 
\gulzar{I am not very comfortable with language/terms of IMC and may be using many alternating terms such as web app, resources and so on. I hope we can make it consistent in the final version.}

\textbf{Proposed Approach.}
We conduct a large-scale measurement study of mixing advertising and tracking resources with functional resources using hierarchical analysis at multiple levels of granularity. 
%
Motivated by the success of SPFL in fault-code localization, we adapt SPFL to classify web application's resources into tracking/advertising and functional, implicitly localizing the resources most \emph{likely} to trigger tracking behavior. 
We address the two challenges of adapting SPFL to tracking-inducing code localization with the following insights. 

First, in lieu of designing rigorous tracking tests (i.e., curating several inputs and their expected outputs), we leverage existing filter lists \gulzar{?} to identify a tracking behavior at a terminal point (reflected by a network request to a tracking domain) at page load time.\gulzar{?} 
%
Second, due to the asynchronous nature of today's web applications, a single page-load execution trace may initiate both tracking and functional symptoms. For each of these symptoms, we examine the terminal resources and their entire execution trace, classifying each as tracking or functional. 
%
Lastly, instead of naively collecting execution profiles at the most fine-grained level, we perform this analysis in a hierarchical manner with increasing granularity, i.e., domain, hostname, script, method,  and call stack. Consequently, we precisely target only the resources that are likely to be both tracking and functional before phasing into the  finer-granularity. 
%

We realize our tracking-inducing resource localization approach in a Google Chrome extension. When applied on a web-application, the extension returns a precise set of resources, at increasing granularity level, that are (1) solely tracking inducing, (2) solely functional inducing , or (3) both tracking and functional inducing.


\gulzar{Hadi: Please add the results paragraph. Write about the experimental setting and then dive into most important results. }

%

- measurement: hierarchical granularity analysis

- approach: to debloat ad/tracking methods from bundled scripts

-- For Gulzar to add details


\textbf{Key Contributions.}


%Notes for mself(Gulzar): Introduce Spectra fault localization in SE, compare teh problem statement and match it with the paper's PS. Define objective fucntion and differences and how things are different in two domains. Challanges in this area if applied as is. Insight: 1.Availability of oracle via privacy list. 2.program state level spectra. 3. Three-tier guided search into the program elements, if we don't do that then coverage instrumentation at finest-grained will be extremely expensive. 

\begin{table}[h]
    \centering
    \footnotesize
    \caption{\hl{Analyzing the domains and resources fetched by top tracking scripts}}
    \vspace{-0.1in}
    \label{table: tracking_scripts}
\begin{tabularx}{8.5 cm}{|X|X|X|}
\hline
\textbf{Script URL }        & \textbf{Domain Owned by }& \textbf{Comment} \\
\hline
www.google.com\/\-recaptcha\/api.js
& Google, USA &  Google  reCAPTCHA will analyze the way users navigate through the website. \\
\hline
cdn1.neolith.com\-\/wp-includes\/js\-\/jquery\/jquery.js
& Amazon, USA &  \\
\hline
cdn.megadata.co.kr\-\/dist\/prod\/enp\_tracker\-\_self\_hosted.min.js
& Amazon, USA & This script adds google analytic tracking codes to the website. \\
\hline
code.jquery.com\/jquery\-1.12.4.min.js
& Highwinds Network Group, Inc & It distributes advertising assets for leading platforms including Facebook's LiveRail.
 \\
\hline
ajax.googleapis.com\-\/ajax\/libs\/jquery\-\/1.7.2\/jquery.min.js
& Google, USA & Multiple requests to verint.com. Verint Systems is a Melville, New York-based analytics company. \\
\hline
ecostruxureit.com\-\/wp-includes\/js\/jquery\-\/jquery.min.js?ver=3.5.1
& Google, USA &  \\
\hline
s.pinimg.com/ct/core.js
& Akamai , USA &  \\
\hline
consent.cookiebot.com\-\/uc.js
& Akamai , USA & This scripts requests multiple tracker domains including: youtube-nocookie.com, googleadservices.com, doubleclick.net, amazon-adsystem.com, etc. \\
\hline
uploads-ssl.webflow.com\-\/5ee232b0abd8729f392796\-c6\/js\/webflow.da3e401fa.js
& Amazon , USA &  \\
\hline
\end{tabularx}
\vspace{-2.5ex}
\end{table} 
